The Externalities of Exploration and How Data Diversity Helps Exploitation

Online learning algorithms, widely used to power search and content optimization on the web, must balance exploration and exploitation, potentially sacrificing the experience of current users for information that will lead to better decisions in the future. Recently, concerns have been raised about whether the process of exploration could be viewed as unfair, placing too much burden on certain individuals or groups. Motivated by these concerns, we initiate the study of the externalities of exploration - the undesirable side effects that the presence of one party may impose on another - under the linear contextual bandits model. We introduce the notion of a group externality, measuring the extent to which the presence of one population of users impacts the rewards of another. We show that this impact can in some cases be negative, and that, in a certain sense, no algorithm can avoid it. We then study externalities at the individual level, interpreting the act of exploration as an externality imposed on the current user of a system by future users. This drives us to ask under what conditions inherent diversity in the data makes explicit exploration unnecessary. We build on a recent line of work on the smoothed analysis of the greedy algorithm that always chooses the action that currently looks optimal, improving on prior results to show that a greedy approach almost matches the best possible Bayesian regret rate of any other algorithm on the same problem instance whenever the diversity conditions hold, and that this regret is at most $\tilde{O}(T^{1/3})$. Returning to group-level effects, we show that under the same conditions, negative group externalities essentially vanish under the greedy algorithm. Together, our results uncover a sharp contrast between the high externalities that exist in the worst case, and the ability to remove all externalities if the data is sufficiently diverse.

==> sections/appnegative.tex <==
\section{[OBSOLETE!] Proof of Theorem~\ref{thm:twobridgelinucb} in Section~\ref{sec:negative}}

In this section, we prove that LinUCB achieves constant expected
minority regret when run on the minority alone with
$\theta = \thetazero$. The analysis of the expected minority regret of
LinUCB on the full population for $\theta = \thetaone$ is completely
analogous. We omit formal proofs of the $\Omega(\sqrt{T})$ lower
bounds, which follow a similar structure to the one used in the proof
of the general impossibility result in
Section~\ref{sec:impossibility}, and in fact would follow immediately
as a corollary of this result.

The proof makes use of the following concentration bound:


\begin{lemma} \label{lem:badrounds}
Let $C_t$ be the number of $C$ rounds observed in the first $t$ minority rounds
in the two-bridge instance. For any $\delta \in (0, 1)$,
with probability at least $1-\delta$, $C_t \ge 0.9t$ for all $t \ge 760 \log
(T/\delta)$.
\end{lemma}
\begin{proof}
We apply the following form of the Chernoff bound:
\[
  \Pr\b{C_t \le (1-\gamma) \E{C_t}} \le \exp\p{-\frac{\gamma^2}{2} \E{C_t}}.
\]
Setting $\gamma = 1/19$, we get
\begin{align*}
  \Pr\b{C_t \le \frac{9}{10}t} &=
  \Pr\b{C_t \le \p{1 - \frac{1}{19}} \frac{19}{20}t}
  \le \exp\p{-\frac{(1/19)^2}{2} \frac{19}{20} t}
  = \exp\p{-\frac{t}{760}}
  \le \frac{\delta}{T}
\end{align*}
for $t \ge 760 \log (T/\delta)$. Applying a union bound over all $T$ rounds, we have $C_t
\ge 0.9t$ for all $t \ge 760 \log(T/\delta)$ with probability at least
$1-\delta$.
\end{proof}

Now, consider LinUCB run on the minority population alone on the
two-bridge instance with $\theta = \thetazero$. Since we are
considering running LinUCB on the minority only, majority rounds are
irrelevant, so throughout this proof we abuse notation and use
$t \in \{1, \cdots, T_0\}$ for some $T_0 \leq T$ to index minority
rounds. $T$ is still the total number of (minority plus majority)
rounds.

  This proof heavily exploits the special structure of the two-bridge
  instance to simplify the analysis of LinUCB.  In particular, we
  exploit the fact that the only contexts ever available are the basis
  vectors $[1 ~ 0]\tran$ and $[0 ~ 1]\tran$.  This implies that the
  covariance matrix $Z_t$ is always diagonal, which greatly simplifies
  the expression for the chosen action in
  Equation~\eqref{eq:linucb_def}.  The optimistic estimate of the
  reward for choosing the $i$th basis vector is simply
  \begin{align}
    UCB_i^t := (\thetahatt)_i + f(t)/\sqrt{(Z_t)_{ii}} .
    \label{eq:ucbdef}
  \end{align}
  Additionally, in this special case,  $(Z_t)_{ii}$ is simply the
  number of times that the $i$th basis vector was chosen over the
  first $t$ minority rounds, and $(\thetahatt)_i$ is the average reward
  observed over the $(Z_t)_{ii}$ rounds on which it was chosen.

  Using this fact, we can apply concentration bounds to bound the
  difference between each $(\thetahatt)_i$ and $\theta_i$. Since rewards
  were assumed to be $1$-subgaussian,
  Lemma~\ref{lem:hoeffding} and a union bound give us that for any
  $\delta_1$, for any $t$, with probability at least $1-4\delta_1$, for all $i
  \in \{1,2\}$,
  \begin{align}
    \left\vert \theta_i - \thetahatti \right\vert \le
        \sqrt{2 \log (\tfrac{1}{\delta_1})/(Z_t)_{ii}}
  \label{eq:ucbbound}
\end{align}

Let $B_t$ and $C_t$ be the number of $B$ and $C$ rounds respectively
before round $t$. By Lemma~\ref{lem:badrounds}, for any $\delta_2$,
with probability $1-\delta_2$, $C_t \ge 9 B_t$ when
$t \ge 760 \log(T/\delta_2)$.  Suppose this is the case.  Since it is
only possible to choose $[1 ~ 0]$ on $B$ rounds, we have
$(Z_t)_{11} \leq B_T$. Similarly, since the algorithm can only choose
$[0 ~ 1]$ on every $C$ round, $(Z_t)_{22} \geq C_T \geq 9 B_T$.
Fixing $\delta_1 = 1/\sqrt{T}$ and using the assumption that
$f(t) \geq 2\sqrt{\log(T)}$, Equations~\eqref{eq:ucbdef}
and~\eqref{eq:ucbbound} then imply that for any $t \geq 760
\log(T/\delta_2)$, with probability at least $1-2\delta_1 = 1 -2\sqrt{T}$,
\begin{align*}
  UCB_1^{t}
  &\ge \theta_1 - \sqrt{\frac{2 \log (\sqrt T)}{(Z_t)_{11}}}+
  \frac{f(t)}{\sqrt{(Z_t)_{11}}}
  \ge \frac{1}{2} + \frac{1}{2}\frac{f(t)}{\sqrt{B_t}} ,
\end{align*}
and similarly,
\begin{align*}
  UCB_2^{t}
  &\le \theta_2 + \sqrt{\frac{2 \log (\sqrt{T})}{(Z_t)_{22}}} +
  \frac{f(t)}{\sqrt{(Z_t)_{22}}}
 \le \frac{1}{2} - \varepsilon   +\frac{3}{2}\frac{f(t)}{\sqrt{C_T}}
\le  \frac{1}{2} +\frac{1}{2}\frac{f(t)}{\sqrt{B_T}} \leq UCB_1^{t}.
\end{align*}


This shows that with probability at least $1-\delta_2$, after the
first $760 \log (T/\delta_2)$ rounds, LinUCB picks $[1 ~ 0]\tran$ on
each $B$ round with probability at least $1-2\delta_1$, leading to
zero regret on that round.  To turn this into a bound on expected
regret, first note that with at most $\delta_2$ probability, the
argument above fails to hold, in which case the minority regret is
still bounded by $\varepsilon B_T \leq \varepsilon T$.  When the argument
above holds, LinUCB may suffer up to $\varepsilon$ regret on each of the
first $760 \log (T/\delta_2)$ minority rounds.  On each additional
round, there is a failure probability of $2\delta_1$, and in this case
LinUCB again suffers regret of at most $\varepsilon$.  Putting this
together and setting $\delta_2 = 1/\sqrt{T}$, we get that the expected
regret is bounded by
$\delta_2 \varepsilon T
+ 760 \log(T/\delta_2) \varepsilon
+ 4\delta_1 \varepsilon T
= O(1)$.

\section{Proof of Theorem~\ref{thm:indistinguishability} in Section~\ref{sec:negative}}

  Fix any algorithm $\mathcal{A}$. We will first derive an
  $\Omega(\sqrt{T})$ lower bound on the expected regret of
  $\mathcal{A}$ conditioned on the number of
  $B$ rounds, $B_T$, being large. To complete the proof, we then show
  that $B_T$ is large
  with high probability.

  Let $h_t = \{(x_{1,\tau}, x_{2,\tau}, a_\tau, r_\tau)\}_{\tau=1}^t$ be a
  history of all context vectors, chosen actions, and rewards up to
  round $t$, with $h_0 = \emptyset$. Running $\mathcal{A}$ on the
  two-bridge instance with $\theta = \thetazero$ induces a
  distribution over histories $h_T$. Let $P$ denote the conditional
  distribution of these histories, conditioned on the event that $B_T
  \geq T/800$.  That is, we define
\[
P(h_T) := \Pr\left[h_T \left\vert \theta = \thetazero, B_T \geq
    T/800 \right.\right].
\]
  Similarly, we define
\[
Q(h_T) := \Pr\left[h_T \left\vert \theta = \thetaone, B_T \geq
    T/800 \right.\right].
\]

We first show that $\kl{P(h_T)}{Q(h_T)}$ is upper bounded a constant
that does not depend on $T$.
By the
  chain rule for KL divergences, since $r_t$ is independent of any
  previous contexts, actions, or rewards conditioned on $x_t$,
\begin{align*}
  \kl{P(h_T)}{Q(h_T)}
   =
  & \sum_{t=1}^T \Exp_{h_{t-1} \sim P}[\kl{P((x_{1,t}, x_{2,t}, a_t) \given
    h_{t-1})}{Q((x_{1,t}, x_{2,t}, a_t) \given h_{t-1})}] \\
  & + \sum_{t=1}^T \Exp_{(x_{1,t}, x_{2,t}, a_t) \sim P} [\kl{P(r_t \given x_{1,t}, x_{2,t}, a_t)}{Q(r_t
    \given (x_{1,t}, x_{2,t}, a_t))}] .
\end{align*}
Since the choice of context vectors available at time $t$ is
independent of the value of the parameter $\theta$ and $\mathcal{A}$
may only base its choices on the observed history and current choice
of contexts, it is always the case that
$P((x_{1,t}, x_{2,t}, a_t) \given h_{t-1}) = Q((x_{1,t}, x_{2,t}, a_t)
\given h_{t-1})$, so the first sum in this expression is equal to 0.

To bound the second sum, we make use of the assumption that
$r_t \in \{0,1\}$ for all $t$.\footnote{If we instead assumed rewards
  had Gaussian noise with variance $\sigma^2$, we would have
  $\kl{P_t(r_t \given x_{1,t}, x_{2,t}, a_t)}{Q_t(r_t \given x_{1,t}, x_{2,t}, a_t)} =
  \varepsilon^2/(2\sigma^2)$, and the proof would
  still go through.} Lemma~\ref{lem:bern_kl} then tells us that for
any round $t$,
$\kl{P(r_t \given x_{1,t}, x_{2,t}, a_t)}{Q(r_t \given x_{1,t}, x_{2,t}, a_t)} \le 7 \varepsilon^2/2$
since the probability of getting reward 1 conditioned on a chosen
context is always either $1/2$ or $1/2 - \varepsilon$. Putting this
together, we get that \[
  \kl{P(h_T)}{Q(h_T)} \le \frac{7\varepsilon^2 T}{2} = \frac{7}{2}.
\]

Now, let $E$ be the event that the algorithm $\mathcal{A}$ chooses arm
2 on at least half of the $B$ rounds, conditioned on $B_T \ge T/800$. If $E$ occurs when
$\theta = \thetazero$, the regret of $\mathcal{A}$ is at least
$B_T \varepsilon / 2$, which is on the order of $\sqrt{T}$ when
$B_T \geq T /800$. If $E$ does not occur (i.e., $\overline{E}$ occurs)
when $\theta = \thetaone$, $\mathcal{A}$ again has regret at least
$B_T \varepsilon / 2$. We will use the bound on KL
divergence to show that one of these bad cases happens with high
probability.

By Lemma~\ref{lem:pinkser},
\[
  P(E) + Q(\overline{E}) \ge \frac{1}{2} e^{-\kl{P(h_T)}{Q(h_T)}} \geq
  \frac{1}{2} e^{-7/2}.
\]

Let $R$ be the regret of $\mathcal{A}$.  We then have that
\begin{align*}
\Exp\left[R \left\vert B_T \geq \frac{T}{800}\right. \right] &= \frac{1}{2} \Exp\left[R \left\vert \theta = \thetazero, B_T \geq \frac{T}{800}\right. \right]
+ \frac{1}{2} \Exp\left[R \left\vert \theta = \thetaone, B_T \geq \frac{T}{800}\right. \right] \\
&\geq \frac{1}{2} \Pr\left[E \left\vert \theta = \thetazero, B_T \geq \frac{T}{800}\right. \right]
  \Exp\left[R \left\vert E, \theta = \thetazero, B_T \geq \frac{T}{800}\right. \right] \\
& \quad + \frac{1}{2} \Pr\left[\overline{E} \left\vert \theta = \thetaone, B_T \geq \frac{T}{800}\right. \right]
  \Exp\left[R \left\vert \overline{E}, \theta = \thetazero, B_T \geq \frac{T}{800}\right. \right] \\
&\geq \frac{1}{2} \left(P(E) + Q(\overline{E})\right) \frac{\sqrt{T}}{1600} \\
&\geq \frac{\sqrt T e^{-\frac{7}{2}}}{6400}.
\end{align*}

It remains to bound the probability that $B_T \geq T/800$. By a Chernoff bound,
\[
  \Pr\b{B_T \le \frac{T}{800}} = \Pr\b{B_T \le \frac{\E{B_T}}{2}} \le
  \exp\p{-\frac{\E{B_T}}{8}} = \exp\p{-\frac{T}{3200}}.
\]
Thus, for any $\delta \in (0,1)$, if $T \ge 3200 \log(1/\delta)$, then with probability at least $1-\delta$, $B_T \ge
T/800$.  In particular, let $\delta = 1/2$.  Then if
$T \geq 3200 \log 2$, we have
\begin{align*}
\Exp[R]
&\geq
\Pr\left[B_T \geq \frac{T}{800} \right]
\Exp\left[R \left\vert B_T \geq \frac{T}{800}\right. \right]
\geq \left(\frac{1}{2}\right) \left(\frac{\sqrt T e^{-\frac{7}{2}}}{6400}\right).
\end{align*}
This completes the proof that the regret of $\mathcal{A}$ is
$\Omega(\sqrt{T})$ on this problem instance.


